Efficient Decomposition of Forman-Ricci Curvature on Vietoris-Rips Complexes and Data Applications

Discrete Forman-Ricci curvature (FRC) is an efficient tool that characterizes essential geometrical features and associated transitions of real-world networks, extending seamlessly to higher-dimensional computations in simplicial complexes. In this article, we provide two major advancements: First, we give a decomposition for FRC that inhently allows a local computations of FRC. Second, we construct a set-theoretical proof enabling an efficient algorithms for the local computation of FRC in Vietoris-Rips (VR) complexes. Our findings open new avenues for geometric computations in VR complexes and highlight an essential yet under-explored aspect of data analysis and visualisation: the geometry underpinning statistical patterns.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
%\newcommand{\creflastconjunction}{, and~}

\usepackage{xcolor,hyperref}
\hypersetup{colorlinks,breaklinks,
            linkcolor=blue,urlcolor=blue,
            anchorcolor=blue,citecolor=blue}

\usepackage{todonotes}

\newcommand{\md}[1]{\textcolor{magenta}{#1}}
\newcommand{\MDcom}[2][noinline]{\todo[#1, color=blue!20!white]{\small \texttt{MD}: #2}}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
%\headers{Efficient computations of Forman-Ricci curvature on filtrations of Vietoris-Rips Complexes}{Danillo Barros de Souza et al}
\headers{F.R.C. in V.R. Complexes and data applications}{D.B.S. et al}
% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{Efficient computations of Forman-Ricci curvature on filtrations of Vietoris-Rips Complexes\thanks{Submitted to the editors DATE.
%\funding{This work was funded by ...}}}
% Suggested by Serafim: 
%Efficient decomposition of Forman-Ricci curvature for Vietoris-Rips complexes: Applications to data
\title{Efficient Decomposition of Forman-Ricci Curvature on Vietoris-Rips Complexes and Data Applications
\thanks{This manuscript is for review purposes only.
\funding{This research is supported by the grant\newline PID2023-146683OB-100 funded by MICIU/AEI /10.13039/501100011033 and by\newline ERDF, EU. Additionally, it is supported by Ikerbasque Foundation and the Basque Government through the BERC 2022-2025 program and by the Ministry of Science and Innovation: BCAM Severo Ochoa accreditation CEX2021-001142-S / MICIU / AEI / 10.13039/501100011033. Moreover, the authors acknowledge the financial support received from BCAM-IKUR, funded by the Basque Government by the IKUR Strategy and the European Union NextGenerationEU/PRTR. We also acknowledge the support of ONBODY no. KK-2023/00070 funded by the Basque Government through ELKARTEK Programme. Weiqiang Sun and Mengjun Ding are supported by the National Key Research and Development Project of China under Grant 2024YFB2908301 and by the National Natural Science Foundation of China (NSFC) under Grant 62331017}}}
% Authors: full names plus addresses.
\author{Danillo Barros de Souza\thanks{Basque Center for Applied Mathematics
  (\email{danillo.dbs16@gmail.com})}
  \and Jonatas Teodomiro\thanks{Universidade Federal de Pernambuco (\email{jonatas.teodomiro@ufpe.br})}
  \and Fernando A. N. Santos\thanks{Dutch Institute for Emergent Phenomenal (\email{f.a.nobregasantos@uva.nl})}
  \and
  Mengjun Ding\thanks{School of
  Electronic Information and Electrical Engineering,
  Shanghai Jiao Tong University, Shanghai, China (\email{mengjun\_ding@sjtu.edu.cn})}
  \and
  Weiqiang Sun\thanks{School of
  Electronic Information and Electrical Engineering,
  Shanghai Jiao Tong University, Shanghai, China (\email{sunwq@sjtu.edu.cn})}
  \and
  Mathieu Desroches\thanks{Inria, Montpellier, France (\email{mathieu.desroches@inria.fr
  })}
  \and J\"urgen Jost\thanks{Max Planck Institute for Mathematics in the Sciences, Leipzig,  and Center for Scalable Data Analytics and Artificial Intelligence, Leipzig University, Germany,  and Santa Fe Institute, New Mexico, USA
  (\email{jost@mis.mpg.de}).}
  \and Serafim Rodrigues\thanks{Basque Center for Applied Mathematics (\email{srodrigues@bcamath.org})}}

\usepackage{amsopn}
\usepackage{cleveref}
\DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
